Computational Complexity of Learning Efficiently Generatable Pure States

Understanding the computational complexity of learning efficient classical programs in various learning models has been a fundamental and important question in classical computational learning theory. In this work, we study the computational complexity of quantum state learning, which can be seen as a quantum generalization of distributional learning introduced by Kearns et.al [STOC94]. Previous works by Chung and Lin [TQC21], and B\u{a}descu and O$'$Donnell [STOC21] study the sample complexity of the quantum state learning and show that polynomial copies are sufficient if unknown quantum states are promised efficiently generatable. However, their algorithms are inefficient, and the computational complexity of this learning problem remains unresolved. In this work, we study the computational complexity of quantum state learning when the states are promised to be efficiently generatable. We show that if unknown quantum states are promised to be pure states and efficiently generateable, then there exists a quantum polynomial time algorithm $A$ and a language $L \in PP$ such that $A^L$ can learn its classical description. We also observe the connection between the hardness of learning quantum states and quantum cryptography. We show that the existence of one-way state generators with pure state outputs is equivalent to the average-case hardness of learning pure states. Additionally, we show that the existence of EFI implies the average-case hardness of learning mixed states.

==> Sec_Cryptography.tex <==
\section{Quantum Cryptographic Primitives}
In this section, we introduce quantum cryptographic primitives, which we will use in this work.
Note that throughout this work, as adversaries, we consider uniform QPT algorithms instead of non-uniform QPT algorithms.
\paragraph{One-way state generators.}
In this work, we consider two definitions of OWSGs.
The first one is an original definition of OWSGs introduced by Morimae and Yamakawa~\cite{Crypto:MY22}, which we call projective OWSGs with pure state outputs.
\begin{definition}[Projective OWSGs with Pure State Outputs~\cite{Crypto:MY22}]\label{def:owsg_pure}
    A projective one-way state generator with pure state outputs is a set of uniform QPT algorithms $\Sigma\seteq(\keygen,\StateGen)$ such that:
\begin{itemize}
    \item[$\keygen(1^\secp)$:]
    It takes a security parameter $1^\secp$, and outputs a classical string $k$.
    \item[$\StateGen(1^\secp,k)$:]
    It takes a security parameter $1^\secp$ and $k$, and outputs a pure quantum state $\ket{\psi_k}$.
\end{itemize}
\paragraph{Security.}
We consider the following security experiment $\mathsf{Exp}_{\Sigma,\cA}(1^\secp)$.
\begin{enumerate}
    \item The challenger samples $k\la\keygen(1^\secp)$.
    \item $\cA$ can receive arbitrary polynomially many copies of $\ket{\psi_k}$.
    \item $\cA$ outputs $k^*$.
    \item The challenger measures $\ket{\psi_k}$ with $\{\ket{\psi_{k^*}}\bra{\psi_{k^*}}, I-\ket{\psi_{k^*}}\bra{\psi_{k^*}}\}$.
    \item The experiment outputs $1$ if the result is $\ket{\psi_{k^*}}\bra{\psi_{k^*}}$, and $0$ otherwise.
\end{enumerate}
We say that a projective OWSGs with pure state outputs satisfies security if, for any uniform QPT adversaries,
\begin{align}
    \Pr[\mathsf{Exp}_{\Sigma,\cA}(1^\secp)=1]\leq \negl(\secp).
\end{align}
\end{definition}
\begin{remark}
    We often omit the security parameter $1^\secp$ of $\StateGen(1^\secp,k)$ when it is clear from the context.
\end{remark}
\begin{remark}
    We also consider weak OWSGs (with pure state outputs), where for some polynomial $p$, it satisfies the following $p$-security instead of the standard security above.
    \paragraph{$p$-security}
    For any uniform QPT algorithm $\cA$ and any polynomial $t(\cdot)$,
    \begin{align}
\Pr[\top\la\Vrfy(1^\secp,k^*,\psi_k):k\la\keygen(1^\secp),\psi_k\la\StateGen(1^\secp,k),k^*\la\cA(\psi_k^{\otimes t(\secp)})]\leq 1-p(\secp)
    \end{align}
    for all sufficiently large security parameters $\secp\in\N$.
\end{remark}



After the \cite{Crypto:MY22}, they generalize the definition of OWSGs in this work~\cite{Eprint:MY22}.
As the second definition of OWSGs, we consider their generalized definition of OWSGs
\begin{definition}[OWSGs~\cite{Eprint:MY22}]
A one-way state generator is a set of uniform QPT algorithms $\Sigma\seteq(\keygen,\StateGen,\Vrfy)$ such that:
    \begin{itemize}
    \item[$\keygen(1^\secp)$:] It takes a security parameter $1^\secp$, and outputs a classical string $k$.
    \item[$\StateGen(1^\secp,k)$:] It takes a security parameter $1^\secp$ and $k$, and outputs a quantum state $\psi_k$.
    \item[$\Vrfy(1^\secp,k,\psi)$:]It takes a security parameter $1^\secp$, $k$ and $\psi$, and outputs $\top$ or $\bot$. 
\end{itemize}

\paragraph{Correctness.}
We have
\begin{align}
\Pr[\top\la\Vrfy(1^\secp,k,\psi_k):k\la\keygen(1^\secp),\psi_k\la\StateGen(1^\secp,k)]\geq 1-\negl(\secp).
\end{align}
\paragraph{Security.}
For any uniform QPT algorithms $\cA$ and any polynomials $t(\cdot)$,
\begin{align}
\Pr[\top\la\Vrfy(1^\secp,k^*,\psi_k):k\la\keygen(1^\secp),\psi_k\la\StateGen(1^\secp,k),k^*\la\cA(\psi_k^{\otimes t(\secp)})]\leq \negl(\secp).
\end{align}
\end{definition}
\begin{remark}
    We often omit the security parameter $1^\secp$ of $\StateGen(1^\secp,k)$ and $\Vrfy(1^\secp,k,\psi)$ when it is clear from the context.
\end{remark}

\if0
\begin{definition}[OWSGs with Pure State Outputs]\label{def:owsg_pure}
    A one-way state generator (OWSG) with pure state outputs is a set of uniform QPT algorithms $\Sigma\seteq(\keygen,\StateGen,\Vrfy)$ such that:
\begin{itemize}
    \item[$\keygen(1^\secp)$:] It takes a security parameter $1^\secp$, and outputs a classical string $k$.
    \item[$\StateGen(1^\secp,k)$:] It takes a security parameter $1^\secp$ and $k$, and outputs a pure quantum state $\ket{\psi_k}$.
    \item[$\Vrfy(1^\secp,k,\psi)$:]It takes a security parameter $1^\secp$, $k$ and $\psi$, and outputs $\top$ or $\bot$. 
\end{itemize}

\paragraph{Correctness.}
We have
\begin{align}
\Pr[\top\la\Vrfy(1^\secp,k,\ket{\psi_k}):k\la\keygen(1^\secp),\ket{\psi_k}\la\StateGen(1^\secp,k)]\geq 1-\negl(\secp).
\end{align}
\paragraph{Security.}
For any uniform QPT algorithm $\cA$ and any polynomial $t(\cdot)$,
\begin{align}
\Pr[\top\la\Vrfy(1^\secp,k^*,\ket{\psi_k}):k\la\keygen(1^\secp),\ket{\psi_k}\la\StateGen(1^\secp,k),k^*\la\cA(\ket{\psi_k}^{\otimes t(\secp)})]\leq \negl(\secp).
\end{align}
\end{definition}
\begin{remark}
    We also consider weak OWSGs (with pure state outputs), where for some polynomial $p$, it satisfies the following $p$-security instead of the standard security above.
    \paragraph{$p$-security}
    For any uniform QPT algorithm $\cA$ and any polynomial $t(\cdot)$,
    \begin{align}
\Pr[\top\la\Vrfy(1^\secp,k^*,\psi_k):k\la\keygen(1^\secp),\psi_k\la\StateGen(1^\secp,k),k^*\la\cA(\psi_k^{\otimes t(\secp)})]\leq 1-p(\secp)
    \end{align}
    for all sufficiently large security parameters $\secp\in\N$.
\end{remark}
\fi

\begin{theorem}[\cite{Eprint:MY22}]\label{thm:amp_owsg}
    For all inverse polynomial $p$, $p$-secure OWSGs with pure state outputs exist if and only if OWSGs with pure state outputs exist.
    Similarly, for all inverse polynomial $p$, $p$-secure projective OWSGs with pure state outputs exist if and only if projective OWSGs with pure state outputs exist.
\end{theorem}

\begin{theorem}[\cite{Eprint:HKNY23}]\label{thm:owsg_perfect}
If there exist OWSGs, then OWSGs with perfect correctness exist.
In an OWSG scheme $\Sigma=(\keygen,\StateGen,\Vrfy)$ with perfect correctness, it additionally satisfies the following correctness property.
\begin{align}
\Pr[\top\la\Vrfy(k,\psi_k):k\la\keygen(1^\secp),\psi_k\la\StateGen(k)]=1.
\end{align}
\end{theorem}





\paragraph{EFI.}
In this work, we also consider EFI.
\begin{definition}[EFI] 
    We call $\{\rho_{b,\secp}\}_{b\in\bit,\secp\in\N}$ a pair of EFI states if it satisfies the following properties:
    \begin{description}
        \item[Efficient Generation:] There exists a uniform QPT algorithm $\cA$ that takes as input $1^\secp$ and $b$, and outputs $\rho_{b,\secp} $.
        \item[Statistically Far:]
        \begin{align}
            F(\rho_{0,\secp},\rho_{1,\secp})\leq \negl(\secp).
        \end{align}
        \item[Computational Indistinguishability:]
        For all uniform QPT algorithms $\cA$,
        \begin{align}
            \abs{\Pr[\cA(\rho_{0,\secp})]-\Pr[\cA(\rho_{1,\secp})]}\leq \negl(\secp).
        \end{align}
    \end{description}
\end{definition}

Morimae and Yamakawa show that the existence of EFI is equivalent to the existence of secret-verifiable and statistically-invertible OWSGs (SV-SI-OWSGs).
\begin{definition}[SV-SI-OWSGs:]
    A SV-SI-OWSG is a set of uniform QPT algorithms $\Sigma\seteq (\keygen,\StateGen)$ such that:
    \begin{description}
        \item[$\keygen(1^\secp)$:] It takes a security parameter $1^\secp$, and outputs a classical string.
        \item[$\StateGen(1^\secp,k)$:] It takes a security parameter $1^\secp$ and $k$, and outputs $\psi_{\secp,k}$. 
    \end{description}
    \paragraph{Statistically Invertibility:}
    There exists a polynomial $p$ such that for any $(k,k^*)$ with $k\neq k^*$,
    \begin{align}
        \mathsf{TD}(\psi_{\secp,k},\psi_{\secp,k^*}) \leq 1-2^{-p(\secp)}
    \end{align}
    for all sufficiently large $\secp\in\N$.
    \paragraph{Computational Non-Invertibility:}
    For any uniform QPT adversaries $\cA$ and any polynomials $t$,
    \begin{align}
        \Pr[k\la\cA(\psi_{\secp,k}^{\otimes t(\secp)}):k\la\keygen(1^\secp),\psi_{\secp,k}\la\StateGen(1^\secp,k)]\leq \negl(\secp).
    \end{align}
\end{definition}












\paragraph{Pseudorandom Quantum State Generators}
We also consider pseudorandom quantum state generators.
\begin{definition}[Pseudorandom Quantum State Generators]
    A pseudorandom quantum states generator is a uniform QPT algorithm $G$ that takes as input $1^\secp$ and $k\in\bit^{\secp}$, outputs an $m$-qubit quantum state $\ket{\phi_k}$.
    As the security, we require the following: for any polynomial $t$ and uniform QPT adversary $\cA$, there exists a negligible function $\negl$ such that,
    \begin{align}
        \abs{\Pr[1\la\cA\left(\ket{\psi_k}^{\otimes t(\secp)}\right):k\la\bit^{\secp},\ket{\psi_k}\la G(1^\secp,k)]-\Pr[1\la\cA\left(\ket{\theta}^{\otimes t(\secp)}\right):\ket{\psi}\la \mathcal{H}_{m}]}\leq \negl(\secp)
    \end{align}
\end{definition}





\if0
\begin{definition}[$s^*$-Imbalanced Quantum EFID:]
    Let $s^*$ be a function. 
    An $s^*$-imbalanced quantum EFID is a pair of distribution $\{D_n(s,0),D_n(s,1)\}_{n,s\in\N}$ over classical string such that the following holds:
        \paragraph{Efficiency.}
        There exists a quantum polynomial-time algorithm $\mathsf{EFID}$ such that for every $n\in\N$, $s\in\N$, and $b\in\bit$, $\mathsf{EFID}(1^n,s,b)$ statistically simulates $D_n(s,b)$.
        \paragraph{Computational Indistinguishability.}
        There exists a negligible function $\mu(\cdot)$ such that for all quantum polynomial-sized circuits $\cA$, for every $n\in\N$ and every $s\leq s^*(n)$,
        \begin{align}
            \abs{\Pr_{y\la D_n(s,0)}[\cA(y)=1]-\Pr_{y\la D_n(s,1)}[\cA(y)=1]}\leq \mu(n).
        \end{align}
        \paragraph{Statistical Distance.}
        There exists a negligible function $\mu(\cdot)$ such that for every $n$ and every $s\geq s^*(n)$,
        \begin{align}
            \mathsf{SD}(D_n(s,0),D_n(s,1))\geq 1-\mu(n).
        \end{align}
\end{definition}
\begin{theorem}
    If there exist OWSGs with pure output states, then
    there exists a polynomial $p(\cdot)$ and a function $s^*(\cdot)$ such that for all $n\in\N$, $\abs{s^*(n)}\leq \log p(n)$ and $s^*$-imbalanced quantum EFID exists.
\end{theorem}
\fi




\if0
\begin{definition}[OWSGs without Verification]\label{def:owsg_wo_ver}
    A one-way state generator (OWSG) without verification is a set of uniform QPT algorithms $\Sigma\seteq(\keygen,\StateGen)$ such that:
\begin{itemize}
    \item[$\keygen(1^\secp)$:] It takes a security parameter $1^\secp$, and outputs a classical string $k$.
    \item[$\StateGen(1^\secp,k)$:] It takes a security parameter $1^\secp$ and $k$, and outputs a quantum state $\psi_k$.
\end{itemize}
\paragraph{Security.}
We consider the following security experiment.
\begin{enumerate}
    \item The challenger samples $k\la\keygen(1^\secp)$.
    \item $\cA$ receives $\psi_k^{\otimes t(\secp)}$, where $\psi_k\la\StateGen(k)$.
    \item The challenger receives $k^*$ from $\cA$.
    \item The challenger $\top$ with probability $F(\psi_{k^*},\psi_k)$.
\end{enumerate}
We say that OWSGs without verification satisfy $p$ security if for any uniform QPT adversaries $\cA$ and any polynomial $t$,
\begin{align}
    \Pr[\top\la \mbox{ Challenger}]\leq 1/p(\secp)
\end{align}
for all sufficiently large security parameters $\secp\in\N$.
\end{definition}

\begin{proposition}\label{prop:owsg_wo_ver_owsg}
    OWSGs without verification are implied by OWSGs. (\cref{prop:owsg_wo_ver_owsg}).
\end{proposition}


\begin{proposition}\label{prop:owsg_wo_ver_EFI}
    OWSGs without verification are implied by EFI.
\end{proposition}
The proof of \cref{prop:owsg_wo_ver_owsg,prop:owsg_wo_ver_EFI} are given in \cref{sec:app_owsg,sec:app_EFI}, respectively.
\fi


==> Sec_Hardness_Amplification.tex <==
\section{Hardness Amplification of Average-Case Hardness of Pure State Learning (Or How to Strongly Learn Pure State from Weak Pure State Learning)}

\taiga{This is the most non-trivial part, which I consider for now.}
\begin{theorem}\label{thm:hardness_amplification}
    If there exists a family of polynomial-size quantum circuits $\cS=\{\cS_n\}_{n\in\N}$, where fore every $S\in\cS_n$, $S$ is $\poly(n)$-size and takes no input and outputs $\poly(n)$-qubit pure state, a family of efficiently sampleable distribution $\cC_n$ over $\cS_n$ and inverse polynomial $\epsilon$ and $\delta$ such that $\cS$ is $(\epsilon,\delta)$-hard on average under $\cC$, then there exists a family of polynomial-size quantum circuits $\cS^*=\{\cS_n^*\}_{n\in\N}$, where for every $S\in\cS_n^*$, $S$ is $\poly(n)$-size and takes no input and outputs $\poly(n)$-qubit pure state, and efficiently sampleable distribution $\cC_n^*$ over $\cS_n^*$ such that $\cS^*$ is $(2/3,2/3)$-hard on average under $\cC^*$.
\end{theorem}


\begin{proof}[Proof of \cref{thm:hardness_amplification}]
Let $\cS$ be a family of quantum polynomial-size circuits and $\cC$ be an efficiently sampleable distribution over $\cS$ such that $\cS$ is $(\epsilon,\delta)$-hard on average under $\cC$.
From $\cS$ and $\cC$, we construct $\cS^*$ and $\cC^*$ such that $\cS^*=\{\cS_n^*\}_{n\in\N}$ is $(2/3,2/3)$-hard on average under $\cC^*=\{\cC_n^*\}_{n\in\N}$.
We construct $\cS^*$ and $\cC^*$ by parallel repetition.

\begin{description}
    \item[The description of $(\cS_n^*,\cC_n^*)$:]$ $
    \begin{itemize}
        \item \taiga{I have no good idea how to describe $(\cC_n^*,\cS_n^*)$ formally, but $\cC_n^*$ samples $\cS_n$ accoring to $\cC_n$ $n$-times, obtains $\{S_i\}_{i\in[n]} $ in parallel.}
        \item $\cC_n^*$ sample $S_i\la_{\cC_n}\cS_n$ for all $i\in[n]$.
        \item For all $i\in[n]$, let $S_i^*$ be a quatnum circuit that runs $S_i$ $n$-times in parallel. 
        In other words, $S_i^*\seteq  S_i^{\otimes n}$.
        \item $\cC_n^*$ outputs a quantum circuit $\{S_i^*\}_{i\in[n]}$.
    \end{itemize}
\end{description}
For contradiction, assume that $\cS^*$ is not $(2/3,2/3)$-hard on average under $\cC^*$.
From the assumption, there exists a QPT learning algorithm $\cA$ and polynomial $t$ such that
\begin{align}
    \Pr[F\left(\bigotimes_{i\in[n]} \ket{\psi_i}^{\otimes n}, \phi\right)\geq 1/3:
    \begin{array}{ll}
         S_i\la_{\cC_n}\cS_n \mbox{ for } i\in[n] \\
         \ket{\psi_i}\la S_i \mbox{  for  } i\in[n] \\
         C\la\cA(1^n,\bigotimes_{i\in[n]}\ket{\psi_i}^{\otimes nt(n)})\\
         \ket{\phi}\la C
    \end{array}
    ]\geq 1/3
\end{align}
for all sufficiently large $n\in\N$.
From the $\cA$, we construct a QPT learning algorithm $\cB$ such that 
for some appropriate polynomial $\ell(\cdot)$, which we will specify later,
\begin{align}
    \Pr[F(\ket{\psi},\ket{\phi})\geq 1-\epsilon(n):
    \begin{array}{ll}
         S\la_{\cC_n} \cS_n  \\
         \ket{\psi}\la S\\
         C\la\cB(1^n,\ket{\psi}^{\otimes \ell(n)})\\
         \ket{\phi}\la C
    \end{array}
    ]\geq 1- \delta(n)
\end{align}
for all sufficiently large $n\in\N$, which contradicts that $\cS$ is $(\epsilon,\delta)$-hard on average under $\cC$.

Before describing the construction of $\cB$, let us describe sub-protocol $\mathsf{Inverse}_{j,\cA}(\ket{\psi}^{\otimes nt(n)})$.
\begin{description}
    \item[$\mathsf{Inverse}_{j,\cA}(\ket{\psi}^{\otimes nt(n)})$:] $ $
    \begin{enumerate}
        \item Set $\ket{\psi_j}=\ket{\psi}$.
        \item For every $i\in[n]\setminus j$, generate $\ket{\psi_i}^{\otimes nt(n)}$, where $S_i\la_{\cC_n} \cS_n$ and $\ket{\psi_i}\la S_i$.
        \item Run $C\la \cA\left(\bigotimes_{i\in[n]}\ket{\psi_i}^{\otimes nt(n)}\right)$.
        \item Output $C$.
    \end{enumerate}
\end{description}

We describe the construction of $\cB$ as follows.
\begin{enumerate}
    \item $\cB$ receives $\ket{\psi}^{\ell(n)}$, where $\ket{\psi}\la S$ and $S\la_{\cC_n}\cS_n$.
    \item For every $j\in[n]$, $\cB$ works as follows: 
    \begin{itemize}
        \item Run $C_i\la\mathsf{Inverse}_{j,\cA}(\ket{\psi}^{\otimes nt(n)})$ for every $i\in[n]$.
        For every $i\in[n]$, we define a new circuit $C_i[j]$, which is the same as $C_i$ except that $C_i[j]$ traces out all quantum states except for $j$-register.
        Let $\rho_i[j]\la C_i[j]$.
        \item For each $i\in[n]$,
        run $b\la\mathsf{SWAP}(\rho_i[j],\ket{\psi})$ for $n^2$-times, output $X_i[j]=C_i[j]$ if $b=1$ more than $n^2/2$-times, and output $X_i[j]=\bot$ otherwise.
    \end{itemize}
    \item $\cB$ outputs the lexicographically first $X_i[j]$ such that $X_i[j]\neq \bot$.
\end{enumerate}
We analyze the probability that $\cB$ outputs a nice classical description.
First of all, for all $j\in[n]$, we define a set of circuits $\mathsf{Bad}_{j,\cA}\subseteq \cS_n$ as follows.
\begin{align}
    \mathsf{Bad}_{j,\cA}\seteq \left\{S \mid 
    \Pr[F\left(\bigotimes_{i\in[n]} \ket{\psi_i}^{\otimes n},i \phi\right)\geq 1/3:
    \begin{array}{ll}
         \{S_i\}_{i\in[n]\setminus j}\la_{\cC_n}\cS_n \\
         \ket{\psi_i}\la S_i \mbox{  for  } i\in[n]\setminus j \\
         \ket{\psi_j}\la S\\
         C\la\cA(1^n,\bigotimes_{i\in[n]}\ket{\psi_i}^{\otimes nt(n)})\\
         \phi\la C
    \end{array}
    ]\leq 1/6
    \right\}
\end{align}

Now, there is at least one $j\in[n]$ such that
\begin{align}
    \Pr_{S\la_{\cC_n}\cS_n }[S\in \mathsf{Bad}_{j,\cA}]= \sum_{S\in\mathsf{Bad}_{j,\cA}}\Pr[S\la_{\cC_n}\cS_n]\leq ???.
\end{align}
This is justified as follows.
For contradiction assume that for all $j\in [n]$,
\begin{align}
    \Pr_{S\la_{\cC_n}\cS_n }[S\in \mathsf{Bad}_{j,\cA}]\geq ???
\end{align}
Then, we have
\begin{align}
    &\Pr[F\left(\bigotimes_{i\in[n]}\ket{\psi_i},\bigotimes_{i\in[n]}\ket{\phi_i}\right)\geq 1/3:
    \begin{array}{ll}
         \{S_i\}_{i\in[n]}\la_{\cC_n}\cS_n \\
         \ket{\psi_i}\la S_i \mbox{ for } i\in[n]\\
         \{C_i\}_{i\in[n]}\la\cA(1^n,\ket{\psi_i}^{\otimes t(n)})\\
         \ket{\phi_i}\la C_i \mbox{ for } i\in[n]
    \end{array}
    ]\\
    &=\sum_{\{S_i\}_{i\in [n]},\{C_i\}_{i\in[n]}}
    \Pr[\{S_i\}_{i\in[n]}\la_{\cC_n} \cS_n]\Pr[\{C_i\}_{i\in[n]}\la\cA(1^n,\ket{\psi_i}^{\otimes t(n)})]\Pr[F\left(\bigotimes_{i\in[n]}\ket{\psi_i},\bigotimes_{i\in[n]} \ket{\phi_i}\right)\geq 1/3]\\
    &=\sum_{\{S_i\notin \mathsf{Bad}_{i,\cA}\}_{i\in[n]},\{C_{i}\}_{i\in[n]}}\Pr[\{S_i\}_{i\in[n]}\la_{\cC_n} \cS_n]\Pr[\{C_i\}_{i\in[n]}\la\cA(1^n,\ket{\psi_i}^{\otimes t(n)})]\Pr[F\left(\bigotimes_{i\in[n]}\ket{\psi_i},\bigotimes_{i\in[n]} \ket{\phi_i}\right)\geq 1/3]\\
    &+\sum_{ \{\{S_{i}\}_{i\in [n]}\mbox{ s.t }\exists i S_i\in\mathsf{Bad_{i,\cA}}\},\{C_i\}_{i\in[n]}}
    %&+\sum_{\exists i \mbox{ s.t }\mathsf{Bad_{i,\cA}},\{C_i\}_{i\in[n]}}
    %\Pr[\{S_i\}_{i\in[n]}\la_{\cC_n} \cS_n]\Pr[\{C_i\}_{i\in[n]}\la\cA(1^n,\ket{\psi_i}^{\otimes t(n)})]\Pr[F\left(\bigotimes_{i\in[n]}\ket{\psi_i},\bigotimes_{i\in[n]} \ket{\phi_i}\right)\geq 1/3
\end{align}



\end{proof}




































==> Sec_OWSG.tex <==

\section{Proof of \cref{prop:owsg_wo_ver_owsg}}\label{sec:app_owsg}
\begin{definition}[OWSGs]\label{def:owsg}
    A one-way state generator (OWSG) is a set of uniform QPT algorithms $\Sigma\seteq(\keygen,\StateGen,\Vrfy)$ such that:
\begin{itemize}
    \item[$\keygen(1^\secp)$:] It takes a security parameter $1^\secp$, and outputs a classical string $k$.
    \item[$\StateGen(1^\secp,k)$:] It takes a security parameter $1^\secp$ and $k$, and outputs a quantum state $\psi_k$.
    \item[$\Vrfy(1^\secp,k,\psi_k)$:]It takes a security parameter $1^\secp$, $k$ and $\psi_k$, and outputs $\top$ or $\bot$. 
\end{itemize}
\paragraph{Correctness.}
We have
\begin{align}
\Pr[\top\la\Vrfy(1^\secp,k,\psi_k):k\la\keygen(1^\secp),\psi_k\la\StateGen(1^\secp,k)]\geq 1-\negl(\secp).
\end{align}
\paragraph{Security.}
For any non-uniform QPT algorithm $\cA$ and any polynomial $t(\cdot)$,
\begin{align}
\Pr[\top\la\Vrfy(1^\secp,k^*,\psi_k):k\la\keygen(1^\secp),\psi_k\la\StateGen(1^\secp,k),k^*\la\cA(\psi_k^{\otimes t(\secp)})]\leq \negl(\secp).
\end{align}
\end{definition}
\begin{remark}
We say that an OWSG scheme $\Sigma=(\keygen,\StateGen,\Vrfy)$ satisfies perfect correctness if it satisfies the following equation
\begin{align}
\Pr[\top\la\Vrfy(1^\secp,k,\psi_k):\psi_k\la\StateGen(1^\secp,k)]=1
\end{align}
for all $k$.
\end{remark}
We can show that if there exists an OWSG scheme, then there also exists an OWSG scheme with perfect correctness.
\begin{proposition}\label{prop:perfect_owsg}
    If there exists an OWSG scheme, then there also exists an OWSG scheme with perfect correctness.
\end{proposition}
\begin{proof}[Proof of \cref{prop:owsg_wo_ver_owsg}]
    We construct OWSG without verification algorithm $\Sigma^*=(\keygen^*,\StateGen^*)$ from OWSG with perfect correctness $\Sigma=(\keygen,\StateGen,\Vrfy)$.
    $\keygen^*$ and $\StateGen^*$ works in the same way with $\keygen$ and $\StateGen$, respectively.
    Now, we can prove the security of $\Sigma^*$ as follows.
    Assume that $\Sigma^*$ is not secure.
    Then, there exists a non-uniform QPT adversary $\cA$, a polynomial $t$, and $p$ such that
    \begin{align}
        \sum_{k,k^*}\Pr[k\la\keygen(1^\secp)]\Pr[k^*\la\cA(\psi_k^{\otimes t(\secp)})]F(\psi_k,\psi_{k^*})\geq 1/p(\secp).
    \end{align}
If we define 
\begin{align}
    S\seteq\left\{(k,k^*)\mid F(\psi_k,\psi_{k^*})\geq 1/2p(\secp) \right\},
\end{align}
we have
\begin{align}
    \sum_{k,k^*\in S}\Pr[k\la \keygen(1^\secp)]\Pr[k^*\la\cA(\psi_k^{\otimes t(\secp)})]\geq 1/2p(\secp).
\end{align}
Now, we construct a QPT adversary $\cB$ that breaks the security of OWSG as follows:
$\cB$ receives $\psi_k^{\otimes t(\secp)}$, runs $k^*\la \cA(\psi_k^{\otimes t})$, and outputs $k^*$.
Now, we have
\begin{align}
    &\sum_{k,k^*}\Pr[k\la\keygen(1^\secp)]\Pr[k^*\la\cB(\psi_k^{\otimes t(\secp)})] \Pr[\top\la\Vrfy(k^*,\psi_k)]\\
    &=\sum_{k,k^*}\Pr[k\la\keygen(1^\secp)]\Pr[k^*\la\cA(\psi_k^{\otimes t(\secp)})] \Pr[\top\la\Vrfy(k^*,\psi_k)]\\
    &\geq \sum_{k,k^*\in S}\Pr[k\la\keygen(1^\secp)]
    \Pr[k^*\la\cA(\psi_k^{\otimes t(\secp)})] \Pr[\top\la\Vrfy(k^*,\psi_k)]\\
    &\geq\sum_{k,k^*\in S}\Pr[k\la\keygen(1^\secp)]
    \Pr[k^*\la\cA(\psi_k^{\otimes t(\secp)})] \left(\Pr[\top\la\Vrfy(k^*,\psi_{k^*})]- \sqrt{1-1/2p(\secp)}\right)\\
    &\geq 1/8p(\secp)^2.
\end{align}
Here, in the second inequality, we have used that $F(\psi_k,\psi_{k^*})\geq 1/p(\secp)$ for all $k,k^*\in S$, and in the last inequality, we have used that $\Sigma$ satisfies perfect correctness and $\sqrt{1-1/2p(\secp)}\leq 1-1/4p(\secp)$.
This contradicts that $\Sigma$ satisfies security.
Therefore, $\Sigma^*$ satisfies security.
\end{proof}







\section{Proof of \cref{prop:owsg_wo_ver_EFI}}\label{sec:app_EFI}
\begin{definition}[Secret-Verifiable and Statistically-Invertible OWSGs (SV-SI-OWSGs)]
    A secretly-verifiable and statistically-invertible OWSG (SV-SI-OWSG) is a set of QPT algorithms $(\keygen,\StateGen)$ as follows.
\begin{itemize}
    \item[$\keygen(1^\secp)$:] It takes a security parameter $1^\secp$, and outputs a classical string $k$.
    \item[$\StateGen(1^\secp,k)$] It takes as input a security parameter $1^\secp$, and outputs a classical string $k$.
\end{itemize}
\paragraph{Statistical invertibility:}
There exists a polynomial $p$ such that for any $k$ and $k'$ ($k\neq k'$), $\mathsf{TD}(\psi_k,\psi_{k'})\geq 1-\negl(\secp)$.
\paragraph{Computational non-invertibility:}
For any QPT adversary $\cA$ and polynomial $t$,
\begin{align}
    \Pr[k\la\cA(\psi_k^{\otimes t}): k\la\keygen(1^\secp),\psi_k\la\StateGen(1^\secp,k)]\leq \negl(\secp).
\end{align}
\end{definition}



\begin{proof}[Proof of \cref{prop:owsg_wo_ver_EFI}]
We construct OWSG without verification algorithm $\Sigma^*=(\keygen^*,\StateGen^*)$ from SV-SI-OWSGs $\Sigma=(\keygen,\StateGen)$.
$\keygen^*$ and $\StateGen^*$ works in the same way with $\keygen$ and $\StateGen$, respectively.
Now, we can prove the security of $\Sigma^*$ as follows.
For a contradiction, assume that $\Sigma^*$ is not secure.
Then, there exists a non-uniform QPT adversary $\cA$, a polynomial $t$ and $p$ such that
\begin{align}
\sum_{k,k^*}\Pr[k\la\keygen(1^\secp)]\Pr[k^*\la\cA(\psi_k^{\otimes t(\secp)})]F(\psi_k,\psi_{k^*})\geq 1/p(\secp).
\end{align}
Because $\Sigma$ satisfies statistical invertibility, for any $k\neq k^*$, we have
\begin{align}
    F(\psi_k,\psi_{k^*})\leq \negl(\secp).
\end{align}
Therefore, we have 
\begin{align}
    &\sum_{k}\Pr[k\la \keygen(1^\secp)]\Pr[k\la\cA(\psi_k^{\otimes t(\secp)})]
    \geq 1/p(\secp)-\negl(\secp).
\end{align}
Now, we can construct a QPT adversary $\cB$ that breaks the security of $\Sigma$.
$\cB$ receives $\psi_k^{\otimes t(\secp)}$, runs $k^*\la\cA(\psi_k^{\otimes t(\secp)})$, and outputs $k^*$.
Now, we have
\begin{align}
    &\sum_{k,k^*}\Pr[k\la\keygen(1^\secp)]\Pr[k^*\la\cB(\psi_k^{\otimes t(\secp)})]\\
    &=\sum_{k,k^*}\Pr[k\la\keygen(1^\secp)]\Pr[k^*\la\cA(\psi_k^{\otimes t(\secp)})]\\
    &\geq\sum_{k}\Pr[k\la\keygen(1^\secp)]\Pr[k\la\cA(\psi_k^{\otimes t(\secp)})]\geq 1/p(\secp)-\negl(\secp).
\end{align}
This contradicts that $\Sigma$ satisfies security.
\end{proof}





==> Sec_pro_OWSG.tex <==

\section{Proof of \cref{thm:equivalence_pro_owsg}}\label{sec:proof_pro_owsg}
In this section, we prove \cref{thm:equivalence_pro_owsg}.
\cref{thm:equivalence_pro_owsg} directly follows from the following \cref{lem:pro_perf_owsg,lem:standard_perf_owsg}.

\begin{lemma}[\cite{Eprint:MY22}]\label{lem:pro_perf_owsg}
    Projective OWSGs with pure state outputs exist if and only if OWSGs with pure state output, which satisfies perfect correctness.
\end{lemma}
\begin{lemma}[\cite{Eprint:HKNY23}]\label{lem:standard_perf_owsg}
    OWSGs with pure state outputs exist if and only if OWSGs with pure state outputs, which satisfies perfect correctness.
\end{lemma}

\begin{proof}[Proof of \cref{lem:pro_perf_owsg}]
It is trivial to show that if projective OWSGs with pure state outputs exist, then OWSGs with pure state outputs, which satisfies perfect correctness.
In the following, we show the reverse direction.
Let $\Sigma=(\keygen,\StateGen,\vrfy)$ be an OWSG with pure state outputs, which satisfies perfect correctness.
Then, we show that $\Sigma'=(\keygen,\StateGen)$ is projective OWSGs with pure state outputs.
We show the security.
For contradiction, assume that there exists a QPT algorithm $\cA$ that breaks the security of projective OWSGs of $\Sigma'$.
Then, there exists polynomials $t$ and $p$ such that
\begin{align}
    \sum_{k,k^*}\Pr[k\la\keygen(1^\secp)]\Pr[\cA(1^\secp,\ket{\psi_k}^{\otimes t(\secp)})]\abs{\bra{\psi_k}\ket{\psi_{k^*}}}^2\geq 1/p(\secp)
\end{align}
for infinitely many $n\in\N$.
If we define 
\begin{align}
     \mathsf{Good_{\secp}}\seteq \left\{(k,k^*): \abs{\bra{\psi_{k}}\ket{\psi_{k^*}}}^2\geq 1/2p(\secp)\right\},
\end{align}
then we have
\begin{align}
    \sum_{(k,k^*)\in\mathsf{Good}}\Pr[k\la\keygen(1^\secp)]\Pr[\cA(1^\secp,\ket{\psi_k}^{\otimes t(\secp)})]\abs{\bra{\psi_k}\ket{\psi_{k^*}}}^2\geq 1/2p(\secp)
\end{align}
for infinitely many $n\in\N$.




Now, we construct a QPT algorithm $\cB$ that breaks the security of OWSGs of $\Sigma$.
$\cB$ works as follows.
On input $\ket{\psi_k}^{\otimes t(\secp)}$, $\cB$ runs $k'\la\cA\left(\ket{\psi_k}^{\otimes t(\secp)}\right)$, and outputs $k'$.
We compute the success probability of $\cB$.
\begin{align}
    &\Pr[\top\la\Vrfy(k^*,\ket{\psi_k}): \keygen(1^\secp),\ket{\psi_k}\la\StateGen(k),k^*\la\cA\left(\ket{\psi_k}^{\otimes t(\secp)}\right)]\\
    &=\sum_{k,k^*}\Pr[k\la\keygen(1^\secp)]\Pr[k^*\la\cA\left(\ket{\psi_k}^{\otimes t(\secp)}\right)]\Pr[\top\la\Vrfy(k^*,\ket{\psi_k})]\\
    &\geq\sum_{(k,k^*)\in\mathsf{Good}}\Pr[k\la\keygen(1^\secp)]\Pr[k^*\la\cA\left(\ket{\psi_k}^{\otimes t(\secp)}\right)]\Pr[\top\la\Vrfy(k^*,\ket{\psi_k})]\\
    &\geq \sum_{(k,k^*)\in\mathsf{Good}}\Pr[k\la\keygen(1^\secp)]\Pr[k^*\la\cA\left(\ket{\psi_k}^{\otimes t(\secp)}\right)]\left(\Pr[\top\la\Vrfy(k^*,\ket{\psi_{k^*}})]-\sqrt{1-\frac{1}{2p(\secp)}}\right)\\
    &\geq \frac{1}{2p(\secp)}\left(1-\sqrt{1-\frac{1}{2p(\secp)}}\right),
\end{align}
which contradicts that $\Sigma$ is an OWSG with pure state outputs.
Here, in the second inequality, we have used that $\abs{\bra{\psi_k}\ket{\psi_{k^*}}}^2\geq 1/2p(\secp)$ for all $(k,k^*)\in\mathsf{Good}$, and in the final inequality, we have used that $\Sigma$ satisfies perfect correctness and 
\begin{align}
    \sum_{(k,k^*)\in\mathsf{Good}}\Pr[k\la\keygen(1^\secp)]\Pr[\cA(1^\secp,\ket{\psi_k}^{\otimes t(\secp)})]\abs{\bra{\psi_k}\ket{\psi_{k^*}}}^2\geq 1/2p(\secp).
\end{align}
\end{proof}

\begin{proof}[Proof of \cref{lem:standard_perf_owsg}]
    It trivially follows that if there exist OWSGs with pure state outputs, which satisfies perfect correctness, then ones with pure state outputs exist.
    Therefore, we show the reverse direction.
    Let $\Sigma=(\keygen,\StateGen,\Vrfy)$ be an OWSG with pure state outputs.
    We give a construction $\Sigma^*=(\keygen^*,\StateGen^*,\Vrfy^*)$, which satisfies perfect correctness.
    \paragraph{Construction}
    Without loss of generality, $\Vrfy(1^\secp,k,\psi)$ can be considered as the algorithm working in the following way:

For input $(1^\secp,k,\psi)$, run a classical Turing machine $\cM$ on $(1^\secp,k,\abs{\psi})$, obtain $U_{\Vrfy,k}$, append auxiliary state $\ket{0\cdots0}\bra{0\cdots 0}$ to $\psi$, apply a unitary $U_{\Vrfy,k}$ on $\psi\otimes\ket{0\cdots 0}\bra{0\cdots 0} $, and measure the first qubit of $U_{\Vrfy,k}(\psi\otimes\ket{0\cdots 0}\bra{0\cdots 0})U_{\Vrfy,k}^{\dagger}$ with the computational basis and output $\top$ if the measurement result is $1$ and $\bot$ otherwise.
We give our construction $\Sigma^*=(\keygen^*,\StateGen^*,\Vrfy^*)$.

\begin{description}
    \item[$\keygen^*(1^\secp):$]$ $
    \begin{itemize}
        \item Run $k\la\keygen(1^\secp)$.
        \item Output $k^*\seteq k$.
    \end{itemize}
    \item[$\StateGen^*(1^\secp,k^*)$:]$ $
    \begin{itemize}
        \item Parse $k^*=k$. 
        \item Run $ \psi_k\la \StateGen(1^\secp,k)$.
        \item Run $U_{\Vrfy,k}$ on $\psi_k\otimes\ket{0\cdots 0}\bra{0\cdots 0}$, and measures the first qubit of $ U_{\Vrfy,k}\left(\psi_{k} \otimes \ket{0\cdots 0}\bra{0\cdots 0}\right)U_{\Vrfy,k}^{\dagger}$,  in the computational basis, and obtains the measurement result $b$ and post-measurement quantum state $\rho_{b,k}$.
        \begin{itemize}
            \item If the measurement result is $1$, then output $\psi_k^*\seteq U_{\Vrfy,k}^{\dagger}(\ket{1}\bra{1}\otimes \rho_{1,k})U_{\Vrfy,k}\otimes \ket{1}\bra{1}$.
            \item If the measurement result is $0$, then output $\psi_k^*\seteq U_{\Vrfy,k}^{\dagger}(\ket{0}\bra{0}\otimes \rho_{0,k})U_{\Vrfy,k}\otimes \ket{0}\bra{0}$.
        \end{itemize}
    \end{itemize}
    \item[$\Vrfy^*(1^\secp,k^*,\psi^*)$:]$ $
    \begin{itemize}
        \item Parse $k^*=k$ and $\psi^*\seteq \rho\otimes \ket{b}\bra{b}$.
        \item Measure the last bit of $\psi^*$ in the computational basis.
        \begin{itemize}
            \item If $1$ is obtained, then measure the first qubit of $U_{\Vrfy,k}\rho U_{\Vrfy,k}^{\dagger} $ in the computational basis, and output $\top$ if the measurement outcome is $1$ and $\bot$ otherwise.
            \item If $0$ is obtained, then output $\top$.
        \end{itemize}
    \end{itemize}
\end{description}

\begin{proposition}[Perfect Correctness]\label{prop:perfect}
    $\Sigma^*$ satisfies 
    \begin{align}
        \Pr[\top\la\Vrfy^*(1^\secp,k^*,\ket{\psi_{k^*}}):k^*\la\keygen^*(1^\secp),\ket{\psi_{k^*}}\StateGen^*(1^\secp,k^*)]=1
    \end{align}
    for all $\secp\in\N$.
\end{proposition}

\begin{proposition}\label{prop:sec_owsg}
    $\Sigma^*$ satisfies security.
\end{proposition}

\begin{proof}[Proof of \cref{prop:perfect}]
    
\end{proof}



\end{proof}










